Event reconstruction for KM3NeT/ORCA using convolutional neural networks

The KM3NeT research infrastructure is currently under construction at two locations in the Mediterranean Sea. The KM3NeT/ORCA water-Cherenkov neutrino detector off the French coast will instrument several megatons of seawater with photosensors. Its main objective is the determination of the neutrino mass ordering. This work aims at demonstrating the general applicability of deep convolutional neural networks to neutrino telescopes, using simulated datasets for the KM3NeT/ORCA detector as an example. To this end, the networks are employed to achieve reconstruction and classification tasks that constitute an alternative to the analysis pipeline presented for KM3NeT/ORCA in the KM3NeT Letter of Intent. They are used to infer event reconstruction estimates for the energy, the direction, and the interaction point of incident neutrinos. The spatial distribution of Cherenkov light generated by charged particles induced in neutrino interactions is classified as shower- or track-like, and the main background processes associated with the detection of atmospheric neutrinos are recognized. Performance comparisons to machine-learning classification and maximum-likelihood reconstruction algorithms previously developed for KM3NeT/ORCA are provided. It is shown that this application of deep convolutional neural networks to simulated datasets for a large-volume neutrino telescope yields competitive reconstruction results and performance improvements with respect to classical approaches.

==> tex/bibliography_jinst.tex <==
\begin{thebibliography}{99}
	
	\bibitem{2013JHEP...02..082A}
	E. Kh. Akhmedov, S. Razzaque and A. Yu Smirnov, A. Yu,
	\emph{Mass hierarchy, 2-3 mixing and CP-phase with huge atmospheric neutrino detectors},
	\emph{Journal of High Energy Physics} {\bf 2013} (2013) 82.
	
	\bibitem{Aurisano2016}
	A. Aurisano, A. Radovic, D. Rocco, A. Himmel, M. D. Messier, E. Niner, G. Pawloski, F. Psihas, A. Sousa and P. Vahle,
	\emph{A Convolutional Neural Network Neutrino Event Classifier},
	\emph{Journal of Instrumentation} {\bf 11} (2016).
	
	\bibitem{Russakovsky2014}
	O. Russakovsky, J. Deng, H. Su, J. Krause, S. Satheesh, S. Ma, Z. Huang, A. Karpathy, A. Khosla, M. Bernstein, A. C. Berg and L. Fei-Fei,
	arxiv:1409.0575v3.
	
	\bibitem{Adrian-Martinez2016}
	S. Adrián-Martínez et al.,
	\emph{Letter of Intent for KM3NeT 2.0},
	\emph{Journal of Physics G: Nuclear and Particle Physics} {\bf 43} (2016).
	
	\bibitem{Carminati2009}
	G. Carminati, M. Bazzotti, S. Biagi, S. Cecchini, T. Chiarusi, A. Margiotta, M. Sioli and M. Spurio,
	\emph{MUPAGE: a fast atmospheric MUon GEnerator for neutrino telescopes based on PArametric formulas},
	\emph{Proceeding of the 31st ICRC, Lodz, Poland} (2009).
	
	\bibitem{He2015}
	K. He, X. Zhang, S. Ren and J. Sun,
	\emph{Delving Deep into Rectifiers: Surpassing Human-Level Performance on ImageNet Classification},
	arxiv:1409.0575v3.
	
	\bibitem{Ioffe2015}
	S. Ioffe and C. Szegedy,
	\emph{Batch Normalization: Accelerating Deep Network Training by Reducing Internal Covariate Shift},
	arxiv:1502.03167v3.
	
	\bibitem{Kingma2014}
	D. P. Kingma and J. Ba,
	\emph{Adam: A Method for Stochastic Optimization},
	arxiv:1412.6980v9.
	
	\bibitem{epsilon}
	\emph{Tensorflow API documentation},
	URL: https://www.tensorflow.org/api\_docs/python/tf/train/AdamOptimizer.
	
	\bibitem{orcanet}
	M. Moser and S. Reck, \emph{OrcaNet},
	URL: \url{https://github.com/KM3NeT/OrcaNet}.
	
	\bibitem{SK1998}
	Y. Fukuda for The Super-Kamiokande Collaboration,
	\emph{Measurement of the flux and zenith-angle distribution of upward through-going muons by Super-Kamiokande}, \emph{Phys.Rev.Lett.} {\bf 82} (1999).
	
	\bibitem{Breiman2001}
	L. Breiman,
	\emph{Random Forests}, \emph{Machine Learning} {\bf 45} (2001).
	
	\bibitem{Hocker:2007ht}
	A. Hoecker, P. Speckmayer, J. Stelzer, J. Therhaag, E. von Toerne and H. Voss,
	\emph{TMVA: Toolkit for Multivariate Data Analysis}, 
	arxiv:physics/0703039.
	
	\bibitem{ilsvrc2017_talk}
	\emph{ImageNet: Where have we been? Where are we going?},
	URL: \url{http://image-net.org/challenges/talks_2017/imagenet_ilsvrc2017_v1.0.pdf}.
	
	\bibitem{cs231n}
	\emph{Lecture notes on Convolutional Neural Networks, Stanford University, 2016},
	URL: \url{http://cs231n.github.io/convolutional-networks}.
	
	\bibitem{Goodfellow2016}
	I. Goodfellow and Y. Bengio and A. Courville,
	\emph{Deep Learning} (2016).
	
	\bibitem{tensorflow2015-whitepaper}
	M. Abadi et al., 
	\emph{TensorFlow: Large-Scale Machine Learning on Heterogeneous Systems},
	URL: \url{http://tensorflow.org}.
	
	\bibitem{chollet2015keras}
	F. Chollet and others, 
	\emph{Keras},
	URL: \url{https://keras.io}.
	
	\bibitem{JMLR:v15:srivastava14a}
	N. Srivastava, G. Hinton, A. Krizhevsky, I. Sutskever and R. Salakhutdinov,
	\emph{Dropout: A Simple Way to Prevent Neural Networks from Overfitting}, 
	\emph{Journal of Machine Learning Research} {\bf 15} (2014) 1929--1958.
	
	\bibitem{Cuda}
	J. Nickolls, I. Buck, M. Garland and K. Skadron,
	\emph{Scalable Parallel Programming with CUDA}, 
	\emph{Queue} {\bf 6} (2008) 40--53.
	
	\bibitem{10.1093/biomet/27.3-4.310}
	R. C. Geary,
	\emph{The ratio of the mean deviation to the standard deviation as a test of normality}, 
	\emph{Biometrika} {\bf 27} (1935) 3--4.
	
	\bibitem{bib:hofestaedt2017}
	J.~Hofest\"adt,
	\emph{Performance studies for the ORCA neutrino detector}, 
	\emph{Friedrich-Alexander-Universität Erlangen--N\"urnberg, Germany} (2017).
	
	\bibitem{Adrian-Martinez:2016zzs}
	S. Adrián-Martínez and others,
	\emph{Intrinsic limits on resolutions in muon- and electron-neutrino charged-current events in the KM3NeT/ORCA detector}, 
	\emph{Journal of High Energy Physics} {\bf 5} (2017) 8.
	
	\bibitem{HKKM}
	M. Honda and others,
	\emph{Atmospheric neutrino flux calculation using the {NRLMSISE-00} atmospheric model}, 
	\emph{Phys.Rev. D} {\bf 92} (2017) 023004.
	
	\bibitem{Collaboration:2011nsa}
	M. Ageron and others,
	\emph{ANTARES: the first undersea neutrino telescope}, 
	\emph{Nucl. Instrum. Meth.} {\bf A656} (2011) 11--38.
	
	\bibitem{Guest:2018yhq}
	D. Guest, K. Cranmer and D. Whiteson,
	\emph{Deep Learning and its Application to LHC Physics}, 
	\emph{Ann. Rev. Nucl. Part. Sci.} {\bf 68} (2018) 161--181.
	
	\bibitem{Shilon:2018xlp}
	I. Shilon et al.,
	\emph{Application of Deep Learning methods to analysis of Imaging Atmospheric Cherenkov Telescopes data}, 
	\emph{Astropart. Phys.} {\bf 105} (2019) 44--53.
	
	\bibitem{Erdmann:2017str}
	M. Erdmann, J. Glombitza, and D. Walz,
	\emph{A Deep Learning-based Reconstruction of Cosmic Ray-induced Air Showers}, 
	\emph{Astropart. Phys.} {\bf 97} (2018) 46--53.
	
	\bibitem{Huennefeld:2017pdh}
	M. Hunnefeld,
	\emph{Deep Learning in Physics exemplified by the Reconstruction of Muon-Neutrino Events in IceCube}, 
	\emph{PoS} {\bf ICRC 2017} (2017).
	
	\bibitem{Aiello:2018nvl}
	S. Aiello and others,
	\emph{Characterisation of the Hamamatsu photomultipliers for the KM3NeT Neutrino Telescope}, 
	\emph{JINST} {\bf 13} (2018) P05035.
	
	\bibitem{2018arXiv180511604S}
	S. Santurkar, D. Tsipras, A. Ilyas and A. Madry, 
	\emph{How Does Batch Normalization Help Optimization?}, 
	\emph{NeurIPS'18} (2018).
	
	
	% --- Examples
	
%	\bibitem{a}
%	Author, \emph{Title}, \emph{J. Abbrev.} {\bf vol} (year) pg.
%	
%	\bibitem{b}
%	Author, \emph{Title},
%	arxiv:1234.5678.
%	
%	\bibitem{c}
%	Author, \emph{Title},
%	Publisher (year).
	
	
	% Please avoid comments such as "For a review'', "For some examples",
	% "and references therein" or move them in the text. In general,
	% please leave only references in the bibliography and move all
	% accessory text in footnotes.
	
	% Also, please have only one work for each \bibitem.
	
\end{thebibliography}
